A search for ttbar resonances in the lepton plus jets final state with ATLAS using 4.7 fb^-1 of pp collisions at sqrt(s) = 7 TeV

A search for new particles that decay into top quark pairs (ttbar) is performed with the ATLAS experiment at the LHC using an integrated luminosity of 4.7 fb^-1 of proton-proton (pp) collision data collected at a center-of-mass energy sqrt(s)=7 TeV. In the ttbar --> WbWb decay, the lepton plus jets final state is used, where one W boson decays leptonically and the other hadronically. The ttbar system is reconstructed using both small-radius and large-radius jets, the latter being supplemented by a jet substructure analysis. A search for local excesses in the number of data events compared to the Standard Model expectation in the ttbar invariant mass spectrum is performed. No evidence for a ttbar resonance is found and 95% credibility-level limits on the production rate are determined for massive states predicted in two benchmark models. The upper limits on the cross section times branching ratio of a narrow Z' resonance range from 5.1 pb for a boson mass of 0.5 TeV to 0.03 pb for a mass of 3 TeV. A narrow leptophobic topcolor Z' resonance with a mass below 1.74 TeV is excluded. Limits are also derived for a broad color-octet resonance with Gamma/m = 15.3%. A Kaluza-Klein excitation of the gluon in a Randall-Sundrum model is excluded for masses below 2.07 TeV.

==> Acknowledgements.tex <==
\section*{Acknowledgments}
\label{sec:Acknowledgements}

% Acknowledgements for papers with collision data
% Version 1-Apr-2013

We thank CERN for the very successful operation of the LHC, as well as the 
support staff from our institutions without whom ATLAS could not be 
operated efficiently. 

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, 
Australia; BMWF and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, 
Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, 
China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; 
DNRF, DNSRC and Lundbeck Foundation, Denmark; EPLANET, ERC and NSRF, European Union; 
IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, DFG, HGF, MPG and AvH 
Foundation, Germany; GSRT and NSRF, Greece; ISF, MINERVA, GIF, DIP and Benoziyo Center, 
Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO, 
Netherlands; BRF and RCN, Norway; MNiSW, Poland; GRICES and FCT, Portugal; MERYS 
(MECTS), Romania; MES of Russia and ROSATOM, Russian Federation; JINR; MSTD, 
Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; 
MICINN, Spain; SRC and Wallenberg Foundation, Sweden; SER, SNSF and Cantons of 
Bern and Geneva, Switzerland; NSC, Taiwan; TAEK, Turkey; STFC, the Royal 
Society and Leverhulme Trust, United Kingdom; DOE and NSF, United States of 
America. 

The crucial computing support from all WLCG partners is acknowledged 
gratefully, in particular from CERN and the ATLAS Tier-1 facilities at 
TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), 
KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), 
ASGC (Taiwan), RAL (UK) and BNL (USA) and in the Tier-2 facilities 
worldwide. 
%----------------------------------------------


